Multi-modal Motion Prediction using Temporal Ensembling with Learning-based Aggregation

Recent years have seen a shift towards learning-based methods for trajectory prediction, with challenges remaining in addressing uncertainty and capturing multi-modal distributions. This paper introduces Temporal Ensembling with Learning-based Aggregation, a meta-algorithm designed to mitigate the issue of missing behaviors in trajectory prediction, which leads to inconsistent predictions across consecutive frames. Unlike conventional model ensembling, temporal ensembling leverages predictions from nearby frames to enhance spatial coverage and prediction diversity. By confirming predictions from multiple frames, temporal ensembling compensates for occasional errors in individual frame predictions. Furthermore, trajectory-level aggregation, often utilized in model ensembling, is insufficient for temporal ensembling due to a lack of consideration of traffic context and its tendency to assign candidate trajectories with incorrect driving behaviors to final predictions. We further emphasize the necessity of learning-based aggregation by utilizing mode queries within a DETR-like architecture for our temporal ensembling, leveraging the characteristics of predictions from nearby frames. Our method, validated on the Argoverse 2 dataset, shows notable improvements: a 4% reduction in minADE, a 5% decrease in minFDE, and a 1.16% reduction in the miss rate compared to the strongest baseline, QCNet, highlighting its efficacy and potential in autonomous driving.

==> tables/comparison-with-model-and-temporal-ensembling.tex <==
\begin{table}[!ht]
    \caption{Combining Model Ensembling and Temporal Ensembling - This table presents the results of combining model ensembling and temporal ensembling for the Argoverse 2 validation set. The baseline observes 50 past frames to predict 60 future steps (evaluated at intervals [10, 60)).}
    \label{tab:both-ensembling}
    \scriptsize	
    % \begin{tabular}{@{}lccc@{}}
    \begin{tabularx}{\columnwidth}{X >{\hsize=.3\hsize}Y >{\hsize=.3\hsize}Y > {\hsize=.55\hsize}Y}
        \toprule
        % \multirow{3}{*}{Method} & \multicolumn{3}{c}{$K=6$} \\
        % \cmidrule(lr){2-4}
        % & minADE & minFDE & MissRate \\
        Method &  minADE & minFDE & MissRate \\
        \midrule
        {Baseline}  & 0.50 & 0.99 & 10.73\% \\
        {w/ ModelEns}  & 0.50 & 0.98 & 10.20\% \\
        {w/ TempEns}  & 0.48 & 0.94 & 9.57\% \\
        {w/ ModelEns + TempEns}  & \textbf{0.48} & \textbf{0.94} & \textbf{9.52\%} \\
        \bottomrule
    \end{tabularx}
    % \end{tabular}
\end{table}

==> tables/qcnet.tex <==
\begin{figure*}[ht]
\makebox[\textwidth]{\includegraphics[width=\textwidth]{figures/method/qcnet.png}}
\caption{\footnotesize{The overall pipeline of QCNet.}}
\label{fig:qcnet}
\end{figure*}

==> tables/two-types-of-prediction-dataset.tex <==
\begin{figure}[ht]
\includegraphics[height=1.4cm]{figures/related-works/two-types-prediction-dataset-paper.png}
\caption{%The left figure shows a snapshot-based prediction dataset, while the right illustrates a streaming dataset. 
Prediction types in existing datasets can be categorized into: (a)
Snapshot-based prediction, where each snapshot predicts once within a fixed-length segment, evaluated at that specific time instance; (b) Streaming-based prediction, where the model continuously predicts in a data stream.
}
% Predictions in the streaming dataset exhibit a high degree of overlap between consecutive instances.
\label{fig:dataset-comparison}
\end{figure}
